Bayesian Shape Reconstruction and Optimal Guidance for Autonomous Landing on Asteroids

Construction of the precise shape of an asteroid is critical for spacecraft operations as the gravitational potential is determined by spatial mass distribution. The typical approach to shape determination requires a prolonged mapping phase of the mission over which extensive measurements are collected and transmitted for Earth-based processing. This paper presents a set of approaches to explore an unknown asteroid with onboard calculations, and to land on its surface area selected in an optimal fashion. The main motivation is to avoid the extended period of mapping or preliminary ground observations that are commonly required in spacecraft missions around asteroids. First, range measurements from the spacecraft to the surface are used to incrementally correct an initial shape estimate according to the Bayesian framework. Then, an optimal guidance scheme is proposed to control the vantage point of the range sensor to construct a complete 3D model of the asteroid shape. This shape model is then used in a nonlinear controller to track a desired trajectory about the asteroid. Finally, a multi resolution approach is presented to construct a higher fidelity shape representation in a specified location while avoiding the inherent burdens of a uniformly high resolution mesh. This approach enables for an accurate shape determination around a potential landing site. We demonstrate this approach using several radar shape models of asteroids and provide a full dynamical simulation about asteroid 4769 Castalia.

==> AAS_macros.tex <==
% custom macros for AAS paper


\newcommand{\linearize}[3]{\ensuremath{\left. \frac{\partial #1}{\partial #2} \right|_{#3} \delta #2}}
\newcommand{\norm}[1]{\ensuremath{\left\| #1 \right\|}}
\newcommand{\abs}[1]{\ensuremath{\left| #1 \right|}}
\newcommand{\Real}[1]{\ensuremath{\Re \left\{ #1 \right\}}}
\newcommand{\bracket}[1]{\ensuremath{\left[ #1 \right]}}
\newcommand{\braces}[1]{\ensuremath{\left\{ #1 \right\}}}
\newcommand{\parenth}[1]{\ensuremath{\left( #1 \right)}}
\newcommand{\pair}[1]{\ensuremath{\langle #1 \rangle}}
\newcommand{\met}[1]{\ensuremath{\langle\langle #1 \rangle\rangle}}
\newcommand{\refeqn}[1]{(\ref{eqn:#1})}
\newcommand{\reffig}[1]{Fig. \ref{fig:#1}}
\newcommand{\tr}[1]{\mathrm{tr}\ensuremath{\negthickspace\bracket{#1}}}
\newcommand{\trs}[1]{\mathrm{tr}\ensuremath{[#1]}}
\newcommand{\deriv}[2]{\ensuremath{\frac{\partial #1}{\partial #2}}}
\newcommand{\dderiv}[2]{\ensuremath{\frac{\partial^2 #1}{\partial^2 #2}}}
\newcommand{\dderivc}[3]{\ensuremath{\frac{\partial #1}{\partial #2 \partial #3}}}
\newcommand{\diff}[2]{\ensuremath{\frac{d #1}{d #2}}}
\newcommand{\ddiff}[2]{\ensuremath{\frac{d^2 #1}{d #2^2}}}
\newcommand{\dirDiff}[2]{\ensuremath{\mathbf{D}_{#2} #1 \cdot \delta #2}} % directional derivative
\newcommand{\SO}{\ensuremath{\mathsf{SO(3)}}}
\newcommand{\T}{\ensuremath{\mathsf{T}}}
\renewcommand{\L}{\ensuremath{\mathsf{L}}}
\newcommand{\so}{\ensuremath{\mathfrak{so}(3)}}
\newcommand{\SE}{\ensuremath{\mathsf{SE(3)}}}
\newcommand{\se}{\ensuremath{\mathfrak{se}(3)}}
\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\aSE}[2]{\ensuremath{\begin{bmatrix}#1&#2\\0&1\end{bmatrix}}}
\newcommand{\ase}[2]{\ensuremath{\begin{bmatrix}#1&#2\\0&0\end{bmatrix}}}
\newcommand{\D}{\ensuremath{\mathbf{D}}}
\newcommand{\Sph}{\ensuremath{\mathsf{S}}}
\renewcommand{\S}{\Sph}
\newcommand{\J}{\ensuremath{\mathbf{J}}}
\newcommand{\Ad}{\ensuremath{\mathrm{Ad}}}
\newcommand{\intp}{\ensuremath{\mathbf{i}}}
\newcommand{\extd}{\ensuremath{\mathbf{d}}}
\newcommand{\hor}{\ensuremath{\mathrm{hor}}}
\newcommand{\ver}{\ensuremath{\mathrm{ver}}}
\newcommand{\dyn}{\ensuremath{\mathrm{dyn}}}
\newcommand{\geo}{\ensuremath{\mathrm{geo}}}
\newcommand{\Q}{\ensuremath{\mathsf{Q}}}
\newcommand{\G}{\ensuremath{\mathsf{G}}}
\newcommand{\g}{\ensuremath{\mathfrak{g}}}
\newcommand{\Hess}[1]{\ensuremath{\mathrm{Hess} \, #1}}
\newcommand{\refprop}[1]{Proposition \ref{prop:#1}}
\newcommand{\Poincare}{Poincar\'e }
\newcommand{\vecbf}[1]{\bm{#1}}
\newcommand{\vb}[1]{\bm{#1}}
\newcommand{\vh}[1]{\hat{\bm{#1}}}
\newcommand{\slfrac}[2]{\left.#1\middle/#2\right.}

\DeclareSIUnit\px{px}

\newcommand{\vc}[1]{\ensuremath{#1}}

% relative macros
\newcommand{\rpos}{\ensuremath{x_r}}
\newcommand{\rvel}{\ensuremath{v_r}}
\newcommand{\ratt}{\ensuremath{R_r}}
\newcommand{\rdatt}{\ensuremath{\dot{R}_r}}
\newcommand{\rangvel}{\ensuremath{\Omega_r}}
\newcommand{\rhangvel}{\ensuremath{\hat{\Omega}_r}}


==> tags <==
!_TAG_FILE_FORMAT	2	/extended format; --format=1 will not append ;" to lines/
!_TAG_FILE_SORTED	1	/0=unsorted, 1=sorted, 2=foldcase/
!_TAG_PROGRAM_AUTHOR	Darren Hiebert	/dhiebert@users.sourceforge.net/
!_TAG_PROGRAM_NAME	Exuberant Ctags	//
!_TAG_PROGRAM_URL	http://ctags.sourceforge.net	/official site/
!_TAG_PROGRAM_VERSION	5.8	//
Asteroid 4769 Castalia Reconstruction	manuscript.tex	/^\\paragraph{Asteroid 4769 Castalia Reconstruction}$/;"	P
Asteroid 52760 Reconstruction	manuscript.tex	/^\\paragraph{Asteroid 52760 Reconstruction}$/;"	P
Asteroid num 1620	manuscript.tex	/^\\paragraph{Asteroid \\num{1620} Geographos Reconstruction} $/;"	P
Asteroid num 6489	manuscript.tex	/^\\paragraph{Asteroid \\num{6489} Golevka Reconstruction} $/;"	P
Castalia Landing Site Refinement	manuscript.tex	/^\\paragraph{Castalia Landing Site Refinement}$/;"	P
Castalia Landing Site Selection	manuscript.tex	/^\\paragraph{Castalia Landing Site Selection}$/;"	P
Castalia Vertical Descent	manuscript.tex	/^\\paragraph{Castalia Vertical Descent}$/;"	P
Conclusions	manuscript.tex	/^\\section{Conclusions}$/;"	s
Geometric Tracking Control	manuscript.tex	/^\\subsection{Geometric Tracking Control}$/;"	b
High Resolution Mapping	manuscript.tex	/^\\subsection{High-Resolution Mapping}\\label{sec:refinement}$/;"	b
Introduction	manuscript.tex	/^\\section{Introduction}$/;"	s
Landing Site Determination	manuscript.tex	/^\\subsection{Landing Site Determination}$/;"	b
Multi resolution Landing Area Refinement	manuscript.tex	/^\\section{Multi-resolution Landing Area Refinement}\\label{sec:landing_refinement}$/;"	s
Numerical Example	manuscript.tex	/^\\subsection{Numerical Example}$/;"	b
Numerical Examples	manuscript.tex	/^\\subsection{Numerical Examples}$/;"	b
Numerical Examples	manuscript.tex	/^\\subsection{Numerical Examples}\\label{sec:kinematic_exploration}$/;"	b
Optimal Guidance	manuscript.tex	/^\\subsection{Optimal Guidance}$/;"	b
Optimal Guidance for Shape Reconstruction	manuscript.tex	/^\\section{Optimal Guidance for Shape Reconstruction}\\label{sec:explore_asteroid}$/;"	s
Problem Formulation	manuscript.tex	/^\\section{Problem Formulation}\\label{sec:problem}$/;"	s
Spacecraft Dynamical Model	manuscript.tex	/^\\subsection{Spacecraft Dynamical Model}$/;"	b

